Surface Normal Estimation of Tilted Images via Spatial Rectifier

In this paper, we present a spatial rectifier to estimate surface normals of tilted images. Tilted images are of particular interest as more visual data are captured by arbitrarily oriented sensors such as body-/robot-mounted cameras. Existing approaches exhibit bounded performance on predicting surface normals because they were trained using gravity-aligned images. Our two main hypotheses are: (1) visual scene layout is indicative of the gravity direction; and (2) not all surfaces are equally represented by a learned estimator due to the structured distribution of the training data, thus, there exists a transformation for each tilted image that is more responsive to the learned estimator than others. We design a spatial rectifier that is learned to transform the surface normal distribution of a tilted image to the rectified one that matches the gravity-aligned training data distribution. Along with the spatial rectifier, we propose a novel truncated angular loss that offers a stronger gradient at smaller angular errors and robustness to outliers. The resulting estimator outperforms the state-of-the-art methods including data augmentation baselines not only on ScanNet and NYUv2 but also on a new dataset called Tilt-RGBD that includes considerable roll and pitch camera motion.

==> sections/AngularInequalityProof.tex <==
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.4\textwidth]{sections/figures/theorem2.png} 
\end{center}
\caption{Definitions for theorem 1.}
\label{fig:angular_triangle_ineq}
\end{figure} 
\begin{theorem}
Define the following quantities as in Fig.~\ref{fig:angular_triangle_ineq}:
\begin{align*}
\delta &= cos^{-1}(\hat{\mathbf{n}}^T \mathbf{n}^{gt}) \\
\Delta \theta &= cos^{-1}(\frac{(\boldsymbol{\Uppi} \hat{\mathbf{n}})^T (\boldsymbol{\Uppi} \mathbf{n}^{gt})}{\| \boldsymbol{\Uppi} \hat{\mathbf{n}} \| \| \boldsymbol{\Uppi} \mathbf{n}^{gt} \|}) \\
\Delta \phi &= |cos^{-1}(\| \boldsymbol{\Uppi} \hat{\mathbf{n}} \|) -  cos^{-1}(\| \boldsymbol{\Uppi} \mathbf{n}^{gt} \|) | 
\end{align*}
where $\boldsymbol{\Uppi} = \begin{bmatrix}1 & 0 & 0\\ 0 & 1 & 0\end{bmatrix}$ is the projection matrix onto the $xy$-plane. Then we have the following inequality:
\begin{equation}
    \delta \leq \Delta \phi + \Delta \theta \label{eq:triangle_ineq_angular_domain}
\end{equation}
\end{theorem}

\begin{proof}
%
Based on definitions we have the following identities:
%
\begin{align*}
cos(\delta) = \hat{\mathbf{n}}^T \mathbf{n}^{gt} \textnormal{ and }
cos(\Delta \theta) = \frac{(\boldsymbol\Uppi \hat{\mathbf{n}})^T (\boldsymbol\Uppi \mathbf{n}^{gt})}{\| \boldsymbol{\Uppi} \hat{\mathbf{n}} \| \cdot \| \boldsymbol{\Uppi} \mathbf{n}^{gt} \|}
\end{align*}
%
\begin{equation*}
\begin{split}
cos(\Delta \phi) & = cos(cos^{-1}(\| \boldsymbol{\Uppi} \hat{\mathbf{n}} \|) - cos^{-1}(\| \boldsymbol{\Uppi} \mathbf{n}^{gt}) \|) \\
 & = \| \boldsymbol{\Uppi} \hat{\mathbf{n}} \| \cdot \| \boldsymbol{\Uppi} \mathbf{n}^{gt} \| + (\mathbf{n}^{gt} - \boldsymbol{\Uppi}\mathbf{n}^{gt})^T(\hat{\mathbf{n}} - \boldsymbol{\Uppi}\hat{\mathbf{n}})
\end{split}
\end{equation*}
%
Furthermore, note that from $\delta, \Delta \theta \in [0, \pi]$ and $\Delta \phi \in [0, \frac{\pi}{2}]$, we have:
\begin{align}
    sin(\Delta \theta), \ sin(\Delta \phi) \textnormal{ and } cos(\Delta \phi) \geq 0 \label{eq:sttsphicphi_geq_0}
\end{align}
%
We consider 2 cases: 

Case 1: $\Delta \phi + \Delta \theta > \pi \nonumber$ then $\Delta \phi + \Delta \theta > \pi \geq \delta$ hence holds trivially~\eqref{eq:triangle_ineq_angular_domain}

Case 2: $\Delta \phi + \Delta \theta \leq \pi$. From~\eqref{eq:sttsphicphi_geq_0}, we have:
%
\begin{align}
\begin{split}
cos(\Delta \phi + \Delta \theta) = cos(\Delta \phi)&cos(\Delta \theta) \nonumber \\ & -sin(\Delta \phi)sin(\Delta \theta)
\end{split} \nonumber \\
\leq cos(\Delta \phi)&cos(\Delta \theta) \label{eq:cos_ttplus_phi}
\end{align}
where
\begin{align}
cos(&\Delta \phi)cos(\Delta \theta) \nonumber \\ & = (\boldsymbol\Uppi \hat{\mathbf{n}})^T (\boldsymbol\Uppi \mathbf{n}^{gt}) \nonumber \\  & \ \ \ \ \ \ + cos(\Delta \theta) (\mathbf{n}^{gt} - \boldsymbol{\Uppi}\mathbf{n}^{gt})^T(\hat{\mathbf{n}} - \boldsymbol{\Uppi}\hat{\mathbf{n}}) \nonumber \\
& \leq (\boldsymbol\Uppi \hat{\mathbf{n}})^T (\boldsymbol\Uppi \mathbf{n}^{gt}) + (\hat{\mathbf{n}} - \boldsymbol{\Uppi}\hat{\mathbf{n}})^T(\mathbf{n}^{gt} - \boldsymbol{\Uppi}\mathbf{n}^{gt}) \label{eq:costt_leq_1} \\
& = \hat{\mathbf{n}}^T \mathbf{n}^{gt} = cos(\delta) \label{eq:dotproduct}
\end{align}
%
where~\eqref{eq:costt_leq_1} is obtained due to $cos(\Delta \theta) \leq 1$ and $(\hat{\mathbf{n}} - \boldsymbol{\Uppi}\hat{\mathbf{n}})^T(\mathbf{n}^{gt} - \boldsymbol{\Uppi}\mathbf{n}^{gt}) \geq 0$, and~\eqref{eq:dotproduct} is obtained by noticing that $ ((\mathbf{x} - \boldsymbol{\Uppi} \mathbf{x})^T (\boldsymbol{\Uppi} \mathbf{y}) = 0 \ \forall \mathbf{x}, \mathbf{y} \in \mathbb{R}^3)$. 
%
Finally, from~\eqref{eq:cos_ttplus_phi} and case 2 condition, we have:
%
\begin{align*}
& cos(\Delta \phi + \Delta \theta) \leq cos(\delta) \\
\implies & \Delta \phi + \Delta \theta \geq \delta    
\end{align*}
%
The equality happens when $cos(\Delta \theta) = 1$ or $\Delta\theta = 0$.
\end{proof}

==> sections/background.tex <==
\section{Background}
\label{sec:background}
% \hyunsoo{Let's put an exhaustive list of surface normal estimation in terms of method, loss type, regularization, evaluation dataset, and accuracy. If so, how are we going to organize these work?}
\begin{table*}[h!]
\centering
\footnotesize

\resizebox{\textwidth}{!}{\begin{tabular}{l|c|c|c|c|c|c}
\hline
Related Work     & Training data                                            & Testing data  & Losses & Regularization    & Median (\degree)~$\downarrow$ & 11.25\degree~$\uparrow$ \\ \hline\hline
Li et al., \cite{li2015depthnormalcrf}                   & \multirow{8}{*}{NYUDv2}                                             & \multirow{10}{*}{NYUDv2} & $L_2$          & None                          & 27.8                     & 19.6                    \\ \cline{1-1} \cline{4-7} 
% Ladicky et al., \cite{Ladicky2014DiscriminativelySurfaceNormal}                    &                                                                     &                          & Cls.         & None                          & None                        & 22 (approx.)            \\ \cline{1-1} \cline{4-7} 
Chen et al., \cite{Chen2017SurfaceNormalsInTheWilds}                  &                                                                     &                          & $L_2$          & \begin{tabular}[c]{@{}c@{}}Depth consistency\end{tabular}   & 15.78                    & 39.17                   \\ \cline{1-1} \cline{4-7} 
% Wang et al., \cite{wang2015LocalGlobalSurfaceNormal}                   &                                                                     &                          & Cls.         & None                          & 13.8                     & 44.2                    \\ \cline{1-1} \cline{4-7} 
Eigen and Fergus \cite{eigen2015DepthNormalSemanticLabel}                  &                                                                     &                          & $L_2$          & None                          & 13.2                     & 44.4                    \\ \cline{1-1} \cline{4-7} 
SURGE \cite{wang2016surge}                   &                                                                     &                          & $L_2$          & \begin{tabular}[c]{@{}c@{}}Plane consistency\end{tabular}           & 12.17                    & 47.29                   \\ \cline{1-1} \cline{4-7} 
Bansal et al., \cite{bansal2016Marr2D3DalignmentViaSN}                  &                                                                     &                          & $L_2$          & None                          & 12.0                     & 47.9                    \\ \cline{1-1} \cline{4-7} 
GeoNet \cite{Qi_2018_CVPR}                   &                                                                     &                          & $L_2$          & \begin{tabular}[c]{@{}c@{}}Depth consistency\end{tabular} & 11.8                     & 48.4                    \\ \cline{1-2} \cline{4-7} 
Hickson et al., \cite{hickson2019floorsareflat}                    & \begin{tabular}[c]{@{}c@{}}ScanNet\\ SceneNet\\ NYUDv2\end{tabular} &                          & $L_2$          & None                          & None                        & 48.9                    \\ \cline{1-2} \cline{4-7} 
FrameNet \cite{Huang19FrameNet} & ScanNet                                                             &                          & $L_2$          & \begin{tabular}[c]{@{}c@{}}Tangent consistency\end{tabular} & 11.16  & 50.2 \\ \hline
Hickson et al., \cite{hickson2019floorsareflat}                    & \begin{tabular}[c]{@{}c@{}}ScanNet\\ SceneNet\\ NYUDv2\end{tabular} & \multirow{3}{*}{ScanNet} & $L_2$          & None                          & None                        & 50.9                    \\ \cline{1-2} \cline{4-7} 
FrameNet \cite{Huang19FrameNet} & \multirow{2}{*}{ScanNet}                                            &                          & $L_2$          & \begin{tabular}[c]{@{}c@{}}Tangent consistency\end{tabular} & 8.14   & 60.6 \\ \cline{1-1} \cline{4-7} 
Zeng et al., \cite{zeng2019rgbdcompletion}                   &                                                                     &                          & $L_1$              & None                          & 7.468*                  & 65.65*                  \\ \hline
Zhan et al., \cite{zhan2019selfsupervisedLearningDepthSurfacenormal}                   & KITTI                                                               & KITTI                    & $L_2$          & None                          & 19.11                    & 33.6                    \\ \hline
Depth completion \cite{zhang2018deepdepthcompletion}                   & SUNCG                                                               & SUNCG                    & $L_2$          & None                          & 17.28                    & 37.7                    \\ \hline
\end{tabular}}
\vspace{-2mm}
\caption{Surface normal estimation methods and results. All the works take RGB images as input while (*) indicates that the work also takes depth images as input. ($\downarrow/\uparrow$: the lower/higher the better). The median measures the median of angular error (defined in Equation~\eqref{eq:angular_error}) and $11.25\degree$ denotes the robust metric $s_{\xi=11.25\degree}$ (defined in equation~\eqref{eq:evaluation_metric}).} \label{table:related_works_table}
% \vspace{-15mm}
\end{table*}

% Deep neural networks that are designed to predict surface normal vectors have been trained by making use of large annotated datasets in a supervised learning fashion.
% The task of pixel-wise 2.5D surface normal is usually solved via supervised learning.
%
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=0.5\textwidth]{eccv2020kit/sections/figures/NoisyBiasNormal.jpg}
    \end{center}
    \caption{Bias (black squares) and noisy (red squares) surface normal ground truth: (a) RGB image, (b) Surface normal ground truth from multiview reconstructions, (c)/(e) Slant/Tilt angles representation of surface normal, (d)/(f) Histogram of slant/tilt angle over a flat surface (red square).}
    \label{fig:misaligned_normal}
\end{figure}
%

\todos{Section Outline:}
\begin{enumerate}
    \item Related work (should we have a completely separate Related Work section based on Table 1?)
    \item Characteristics and formulation of L2
    \item Robust evaluation metrics
    
\end{enumerate}
A normal estimator $f:\mathcal{R}(\mathcal{I}) \subset \mathds{R}^2 \rightarrow \mathds{S}^2$ takes as input 
2D coordinate $\mathbf{p} = \begin{bmatrix} x & y \end{bmatrix}^{\mathsf{T}} \in \mathcal{R}(\mathcal{I})$ given an image $\mathcal{I}$ and outputs surface normal with two degree of freedoms where $\mathcal{R}(\mathcal{I})$ is the coordinate range of the image $\mathcal{I}$. The normal estimator can be designed with a convolutional neural network where its weights can be learned by leveraging large datasets~\cite{bansal2016Marr2D3DalignmentViaSN, Chen2017SurfaceNormalsInTheWilds, eigen2015DepthNormalSemanticLabel, hickson2019floorsareflat, Huang19FrameNet, li2015depthnormalcrf, Qi_2018_CVPR, wang2016surge, zeng2019rgbdcompletion, zhan2019selfsupervisedLearningDepthSurfacenormal, zhang2018deepdepthcompletion}\footnote{Classification based surface normal learning is not considered as its accuracy is bounded by the class resolution~\cite{Ladicky2014DiscriminativelySurfaceNormal, wang2015LocalGlobalSurfaceNormal}}.

% an RGB image $\mathcal{I}$ and 2D coordinate $\mathbf{p} = \begin{bmatrix} x & y \end{bmatrix}^{\mathsf{T}} \in \mathcal{R}(\mathcal{I})$ in the image, and outputs surface normal $f(\mathbf{p}, \mathcal{I}; \mathbf{w})$ at pixel location $\mathbf{x}$, and $\mathcal{R}(\mathcal{I})$ is the coordinate range of the image $\mathcal{I}$. 


% parametrized by its weights $\mathbf{w}$
%
% The network $f$ can be trained via classification~\cite{Ladicky2014DiscriminativelySurfaceNormal, wang2015LocalGlobalSurfaceNormal} or regression~\cite{bansal2016Marr2D3DalignmentViaSN, Chen2017SurfaceNormalsInTheWilds, eigen2015DepthNormalSemanticLabel, hickson2019floorsareflat, Huang19FrameNet, li2015depthnormalcrf, Qi_2018_CVPR, wang2016surge, zeng2019rgbdcompletion, zhan2019selfsupervisedLearningDepthSurfacenormal, zhang2018deepdepthcompletion}.
%
% The accuracy of classification approaches is bounded by class resolution, which has been shown inferior performance than the regression approaches in recent works (see Table~1). 
% %
% Therefore, in the rest of the paper, we solely focus on discussing regression approaches.
% Specifically, we learn a network model with parameters $\mathbf{w}$ that takes as input an RGB image $\mathcal{I}$ and outputs an estimated normal direction $\mathbf{{n}}_{pred}(\mathbf{p}; \mathbf{w})$ of the 3D surface at every pixel $\mathbf{p} = \begin{bmatrix} x & y \end{bmatrix}^{T}$ in the image $\mathcal{I}$.
%

Two surface normal representations are geometrically equivalent: 3D unit vector $\mathbf{n}=\begin{bmatrix} n_x & n_y & n_z \end{bmatrix}^\mathsf{T}$ and slant-tilt (2D) $\boldsymbol{\Theta}=\begin{bmatrix}\theta & \phi \end{bmatrix}^\mathsf{T}$. While there exists a bijection map for visible surfaces, their implication is different.

%
\todos{Characteristics of L2}
For the 3D unit representation, the normal estimator is learned to minimize the following data loss:
\begin{align}
 \mathcal{L}_\mathbf{n} &= \frac{1}{2N} \sum_{\mathcal{I} \sim \mathcal{D}}
 \sum_{\mathbf{p} \in \mathcal{R}(\mathcal{I})} \| \mathbf{n}_{\mathcal{I}}(\mathbf{p})- \widehat{\mathbf{n}}_{\mathcal{I}}(\mathbf{p}) \|_{2}^{2}\label{eq:mse_loss}\\
 &= \frac{1}{N}\sum_{\mathcal{I} \sim \mathcal{D}}
 \sum_{\mathbf{p} \in \mathcal{R}(\mathcal{I})} 1 - \mathbf{n}_{\mathcal{I}}(\mathbf{p})^{\mathsf{T}}\widehat{\mathbf{n}}_{\mathcal{I}}(\mathbf{p}) \label{eq:traditional_supervised_loss},
\end{align}
where $\widehat{\mathbf{n}}_{\mathcal{I}}(\mathbf{p}) = f(\mathbf{p}; \mathcal{I})$ is the estimated surface normal, $\mathbf{n}_{\mathcal{I}}(\mathbf{p})$ is its ground truth, $\mathcal{D}$ is the set of training data instances, and $N$ is the total number of pixels in training set. The mean squared error (MSE or $L_2$) in Equation~\eqref{eq:mse_loss} measures the Euclidean distance between unit vectors that is equivalent to the cosine similarity loss in Equation~\eqref{eq:traditional_supervised_loss}.
% measures how close the cosine of the angle difference between two vectors is to $1$, which is equivalent to the mean square error (MSE or $L_2$) in Equation~\eqref{eq:mse_loss}. 

The data loss formulated as $L_2$ or cosine similarity is sensitive to outliers. It is in particular critical for learning surface normal in the presence of estimation noise and bias due to noisy point cloud measurements and camera calibration~\cite{zeng2019rgbdcompletion, hickson2019floorsareflat}. 
%
For instance, Figure~\ref{fig:misaligned_normal} illustrates that the surface normal ground truth is (i) mis-aligned with RGB image (black dotted squares) and (ii) noisy (slant and tilt angles have variation of 20$^{\circ}$ and 30$^{\circ}$, respectively) over a flat region (red squares).


% Existing surface normal estimation frameworks~\cite{bansal2016Marr2D3DalignmentViaSN, Chen2017SurfaceNormalsInTheWilds, eigen2015DepthNormalSemanticLabel, hickson2019floorsareflat, Huang19FrameNet, li2015depthnormalcrf, Qi_2018_CVPR, wang2016surge, zhan2019selfsupervisedLearningDepthSurfacenormal, zhang2018deepdepthcompletion} are large built upon  the $L_2$ loss.
% %
% This loss, however, are known to be sensitive to outliers, leading to suboptimal estimate.
% %
% This is in particular critical for surface normal prediction as the ground truth is computed by a first derivative of noisy point cloud measurements, which amplifies the noise level. 
% %
% Further, 3D mesh reconstructions from multiviews RGB-D to suppress noise can introduce a substantial bias across multiple frames (see Figure~\ref{fig:misaligned_normal}).
%
% \begin{figure}
%     \begin{center}
%     \includegraphics[width=0.5\textwidth]{sections/figures/misaligned_normal.png}
%     \end{center}
%     \caption{(Left) RGB image. (Bottom right) Surface normal ground truth from multiview reconstructions. (Top right) Valid ground truth pixel. Red ovals indicate the shape mismatch between RGB and surface normal images.}
%     \label{fig:misaligned_normal}
% \end{figure}
% %
% These issues have been pointed out by recent works of~\cite{zeng2019rgbdcompletion, hickson2019floorsareflat}.
%


%
\todos{Introduce robust evaluation metrics}
For this reason, robust evaluation metrics on the angular error are employed in test data, e.g., the median, the mean ($L_1$) [Equation~\eqref{eq:evaluation_metric_L1}] and the cardinality of a set of the pixels with angular error below threshold $s_{\xi}$ ($L_0$) [Equation~\eqref{eq:evaluation_metric_L0}]:
\begin{align}
    \mathcal{L_\delta} &= \frac{1}{N} \sum_{\mathcal{I} \sim \mathcal{D}}
 \sum_{\mathbf{p} \in \mathcal{R}(\mathcal{I})} \delta_i \label{eq:evaluation_metric_L1}\\
    s_{\xi} 
    &= |\{i \ \ | \ \ \delta_i < \xi \}|, \ \ \xi = 11.25^{\circ}, 22.5^{\circ}, 30^{\circ} \label{eq:evaluation_metric_L0}
\end{align}
where the angular error $\delta_i$ of pixel $\mathbf{p}_i$ is defined as:
\begin{align}
    \delta_i = \cos^{-1}(\mathbf{n}_{\mathcal{I}}(\mathbf{p}_i)^{\mathsf{T}}\widehat{\mathbf{n}}_{\mathcal{I}}(\mathbf{p}_i)), \ \ \ \delta_i \in [0, \pi]. \label{eq:angular_error}
\end{align}
We denote $i$ for each pixel $\mathbf{p}_i$ in the training or testing set. In subsequent sections, we show that Equation~(\ref{eq:evaluation_metric_L1}) can be upper-bounded by the angle loss on the slant-tilt representation, which is approximated by the loss on SATD representation. We defer the relationship between the unit vector representation and error metric to Supplementary. 

% In section 3, we show that using the unit vector representation for surface normal and cosine loss leads to a vanishing gradient in the output layer while our proposed loss, which is closely related to angular error, does not have this issue.
% %
% Furthermore, it is intrinsically robust to outlier and is closely related to how human perceives surface normal.

% Existing surface normal estimation frameworks~\cite{bansal2016Marr2D3DalignmentViaSN, Chen2017SurfaceNormalsInTheWilds, eigen2015DepthNormalSemanticLabel, hickson2019floorsareflat, Huang19FrameNet, li2015depthnormalcrf, Qi_2018_CVPR, wang2016surge, zhan2019selfsupervisedLearningDepthSurfacenormal, zhang2018deepdepthcompletion} are large built upon  the $L_2$ loss.
% %
% This loss, however, are known to be sensitive to outliers, leading to suboptimal estimate.
% %
% This is in particular critical for surface normal prediction as the ground truth is computed by a first derivative of noisy point cloud measurements, which amplifies the noise level. 
%
% Further, 3D mesh reconstructions from multiviews RGB-D to suppress noise can introduce a substantial bias across multiple frames (see Figure~\ref{fig:misaligned_normal}).
% %
% \begin{figure}
%     \begin{center}
%     \includegraphics[width=0.5\textwidth]{sections/figures/misaligned_normal.png}
%     \end{center}
%     \caption{(Left) RGB image. (Bottom right) Surface normal ground truth from multiview reconstructions. (Top right) Valid ground truth pixel. Red ovals indicate the shape mismatch between RGB and surface normal images.}
%     \label{fig:misaligned_normal}
% \end{figure}
% %
% These issues have been pointed out by recent works of~\cite{zeng2019rgbdcompletion, hickson2019floorsareflat}.
% %
% In contrast to the training loss, the standard evaluation metrics employed in surface normal are robust such as the median of angular error and the cardinality of sets of small angular error $s_{\xi}$:
% %
% \begin{align}
%     s_{\xi} = |\{i \ \ \textnormal{   s.t. } |\delta_i| < \xi \}|, \ \ \xi = 11.25^{\circ}, 22.5^{\circ}, 30^{\circ} \label{eq:evaluation_metric}
% \end{align}
% where the angular error $\delta_i$ of pixel $\mathbf{p}_i$ is defined as:
% \begin{align}
%     \delta_i = cos^{-1}(\mathbf{n}_{\mathcal{I}}(\mathbf{p}_i)^{\mathsf{T}}\mathbf{\widehat{n}}(\mathbf{p}_i,\mathcal{I}; \mathbf{w})), \ \ \ \delta_i \in [0, \pi] \label{eq:angular_error}
% \end{align}
% and we have employed short-hand notation $i$ for each pixel $\mathbf{p}_i$ in the training or testing set.
% %
% Robust losses such as $L_1$ and Huber loss~\cite{Huber09} are a viable solution~\cite{zeng2019rgbdcompletion} to handle outlier contaminated ground truth. 
% %
% However, simply replacing $L_1$ to $L_2$ norm in Equation~\eqref{eq:mse_loss} still makes it closely related to the cosine loss (as a tight upper bound).



% For the 3D unit vector representation, the unit normalization is needed to evaluate the to ensure its unit length, an $L_2$-normalization are often applied at the final output layer as follows:
% \begin{equation}
%     \widehat{\mathbf{n}}(\mathbf{p}, \mathcal{I}; \mathbf{w}) = \frac{f(\mathbf{p}, \mathcal{I}; \mathbf{w})}{||f(\mathbf{p}, \mathcal{I}; \mathbf{w}) ||} \in \mathds{S}^2,
% \end{equation}
% where $\widehat{\mathbf{n}}$ is the predicted unit surface normal.

% The network can be trained by employing an annotated dataset $\mathcal{D}$ to minimize a loss: $\mathcal{L} = \mathcal{L}_{\rm data} + \lambda \mathcal{L}_{\rm reg}$ where $\mathcal{L}_{\rm data}$ is the data loss for surface estimation, and $\mathcal{L}_{\rm reg}$ is a regularization loss, e.g., depth self-supervision~\cite{Chen2017SurfaceNormalsInTheWilds, Qi_2018_CVPR}, tangent normal consistency~\cite{Huang19FrameNet}, and plane normal consistency~\cite{wang2016surge}. The data loss can be described by using the following loss function:
% \begin{align}
%  \mathcal{L}_{\rm data} &= \mathcal{L}_{\textnormal{cosine}/L_2} \nonumber \\ &= \frac{1}{N} \sum_{\mathcal{I} \sim \mathcal{D}}
%  \sum_{\mathbf{p} \in \mathcal{R}(\mathcal{I})} 1 - \mathbf{n}_{\mathcal{I}}(\mathbf{p})^{\mathsf{T}}\mathbf{\widehat{n}}(\mathbf{p},\mathcal{I}; \mathbf{w}) \label{eq:traditional_supervised_loss}\\
%  &= \frac{1}{2N} \sum_{\mathcal{I} \sim \mathcal{D}}
%  \sum_{\mathbf{p} \in \mathcal{R}(\mathcal{I})} || \mathbf{n}_{\mathcal{I}}(\mathbf{p})- \mathbf{\widehat{n}}(\mathbf{p},\mathcal{I}; \mathbf{w}) ||_{2}^{2},\label{eq:mse_loss}
% \end{align}
% where $\mathbf{n}_{\mathcal{I}}(\mathbf{p})$ is the ground truth of the surface normal, $N$ is the total number of pixels. The cosine loss in Equation~\eqref{eq:traditional_supervised_loss} measures how close the cosine of the angle difference between two vectors is to $1$, which is equivalent to the mean square error (MSE/$L_2$) in Equation~\eqref{eq:mse_loss} between the ground-truth and the prediction.
%
% Due to this equivalency, we will refer to this loss as either cosine or $L_2$ loss depending on the context.

% Existing surface normal estimation frameworks~\cite{bansal2016Marr2D3DalignmentViaSN, Chen2017SurfaceNormalsInTheWilds, eigen2015DepthNormalSemanticLabel, hickson2019floorsareflat, Huang19FrameNet, li2015depthnormalcrf, Qi_2018_CVPR, wang2016surge, zhan2019selfsupervisedLearningDepthSurfacenormal, zhang2018deepdepthcompletion} are large built upon  the $L_2$ loss.
% %
% This loss, however, are known to be sensitive to outliers, leading to suboptimal estimate.
% %
% This is in particular critical for surface normal prediction as the ground truth is computed by a first derivative of noisy point cloud measurements, which amplifies the noise level. 
% %
% Further, 3D mesh reconstructions from multiviews RGB-D to suppress noise can introduce a substantial bias across multiple frames (see Figure~\ref{fig:misaligned_normal}).
% %
% \begin{figure}
%     \begin{center}
%     \includegraphics[width=0.5\textwidth]{sections/figures/misaligned_normal.png}
%     \end{center}
%     \caption{(Left) RGB image. (Bottom right) Surface normal ground truth from multiview reconstructions. (Top right) Valid ground truth pixel. Red ovals indicate the shape mismatch between RGB and surface normal images.}
%     \label{fig:misaligned_normal}
% \end{figure}
% %
% These issues have been pointed out by recent works of~\cite{zeng2019rgbdcompletion, hickson2019floorsareflat}.
% %
% In contrast to the training loss, the standard evaluation metrics employed in surface normal are robust such as the median of angular error and the cardinality of sets of small angular error $s_{\xi}$:
% %
% \begin{align}
%     s_{\xi} = |\{i \ \ \textnormal{   s.t. } |\delta_i| < \xi \}|, \ \ \xi = 11.25^{\circ}, 22.5^{\circ}, 30^{\circ} \label{eq:evaluation_metric}
% \end{align}
% where the angular error $\delta_i$ of pixel $\mathbf{p}_i$ is defined as:
% \begin{align}
%     \delta_i = cos^{-1}(\mathbf{n}_{\mathcal{I}}(\mathbf{p}_i)^{\mathsf{T}}\mathbf{\widehat{n}}(\mathbf{p}_i,\mathcal{I}; \mathbf{w})), \ \ \ \delta_i \in [0, \pi] \label{eq:angular_error}
% \end{align}
% and we have employed short-hand notation $i$ for each pixel $\mathbf{p}_i$ in the training or testing set.
% %
% Robust losses such as $L_1$ and Huber loss~\cite{Huber09} are a viable solution~\cite{zeng2019rgbdcompletion} to handle outlier contaminated ground truth. 
% %
% However, simply replacing $L_1$ to $L_2$ norm in Equation~\eqref{eq:mse_loss} still makes it closely related to the cosine loss (as a tight upper bound).
% In section 3, we show that using the unit vector representation for surface normal and cosine loss leads to a vanishing gradient in the output layer while our proposed loss, which is closely related to angular error, does not have this issue.
% %
% Furthermore, it is intrinsically robust to outlier and is closely related to how human perceives surface normal.

\noindent\textbf{Regularization} To handle the noisy ground truth data, existing methods leverage geometric self-supervision. %
For example, depth and surface normal can be complementary as the surface normal is the derivative of the depth~\cite{Chen2017SurfaceNormalsInTheWilds, Qi_2018_CVPR}.
%
An orthogonality constraint between the surface normal of a plane and its spanned vectors is exploited in a multitask network that learns to predict depth, surface normal, plane semantics, and edges~\cite{wang2016surge}.
%
Similarly, the labeled plane semantics are used to enforce smoothness on the ground truth surface normal~\cite{hickson2019floorsareflat}.
%
In addition, the cross data (real and synthetic) supervision can be used to lessen the effect of noise and bias~\cite{hickson2019floorsareflat}.
%
FrameNet~\cite{Huang19FrameNet} achieves state-of-the-art in surface normal estimation by (i) post-processing the ground truth data via a robust quadrangulation~\cite{Huang18Quadriflow} and detecting invalid regions of the ground truth; (ii) constraining the surface normal prediction to be consistent with its tangential principle directions; and (iii) employing a high capacity network architecture (e.g., DORN~\cite{fu2018dorn}) with dropout-2D as an extra regularization mechanism.
%
Table~\ref{table:related_works_table} summarizes the existing methods regarding datasets, accuracy, loss function, and regularization methods.

Unlike previous regularization, we use semantic multi-plane instance proposal. Following the idea of PlaneRCNN~\cite{Liu2019planercnn} to detect plane instances, our method does not require to predict edges and depth to apply coplanarity constraints~\cite{wang2016surge}.
%
% Following the idea of PlaneRCNN~\cite{Liu2019planercnn} to detect plane instances using Mask-RCNN~\cite{he2017maskrcnn}, we are not required to predict edges and depth to apply orthogonality constraints~\cite{wang2016surge}. Note that this differs from semantic plane segmentation~\cite{hickson2019floorsareflat} as it allows 
% (in stead of semantic plane segmentation) 
%
Instead, we construct a self-supervised learning framework that can jointly predict plane instances and surface normal while being geometric consistent, i.e., the homogeneity of normal directions on flat surfaces.
% can employ the fact that the surface normal in the plane instance is homogeneous~\cite{hickson2019floorsareflat}.
%
% In stead of using planar semantics to smooth out the ground truth surface normal~\cite{hickson2019floorsareflat}, we construct a network that it can jointly predict plane instances and surface normals while being geometric consistent, i.e., the homogeneity of normal directions on flat surfaces.
%
% In order to keep the planar semantic (flat surfaces) being consistent across different frames with varying orientations, we do not label planes with discrete orientations as proposed in PlaneRCNN~\cite{Liu2019planercnn} (the same plane will have different labels with different cameras' orientations), we in stead just detect which set of pixels constitutes flat surfaces.

==> sections/dataset.tex <==
\section{Dataset}
\label{sec:dataset}
\begin{figure*}[t]
\includegraphics[width=\textwidth]{sections/figures/annotation} 
\centering
\vspace{-5mm}
\caption{We refine the noisy plane annotation. (a) Given a noisy plane instance, (b) we fit a plane using the depth from ScanNet with a strict threshold, which produces a set of sparse yet accurate points. (c) Using the point set, we incrementally grow the planar region based on the surface normal from FrameNet. (d-e) This refinement allows us to precise plane instance labels that can be used to train to enforce plane-normal consistency.}
\label{fig:annotation_cleanup}
\end{figure*}

% \begin{itemize}
%     \item Write up motivations for the misalignment: the indoor datasets such as ScanNet, Matterport3D minimize the human labour by reconstructing 3D environments from RGB-D images, then the experts directly annotate on the 3D reconstructed scene. This annotation is then projected onto 2D images. Due to the estimated poses of each camera as well as the mesh triangulation is degraded over frames, there is a misalignment in a large portions of the dataset. This causes inconsistency in training the network. [REF figure 4 and rephrase the text in figure 4 here].
%     \item Therefore, in this section we propose a simple algorithm to fix this issue and obtain a cleaner planar annotated from the misaligned 3D annotations. 
%     \item Copy algorithm here, polish the previous text
%     \item Add steps for the algorithm, showing it by // - comments in code to match the steps describing in Figure 5. then add text for each step to the figure.
% \end{itemize}

% Misalignment between RGB image and annotations in ScanNet dataset: (Top) The RGB images. (Bottom) The projected 3D annotations on images. The black dotted ovals indicate the object in the original RGB images. The red ovals indicate the corresponding annotated parts of the objects circled in black. We can see that throughout many examples there is a substantial misalignment between objects in RGB image and object in the annotated images.

% \begin{figure*}[h!]
% \includegraphics[width=\textwidth]{sections/figures/rgb_misalignment.png} 
% \centering
% \caption{Misalignment between RGB image and annotations in ScanNet dataset: (Top) The RGB images. (Bottom) The projected 3D annotations overlaid on corresponding RGB images. The dotted circles indicate the objects' positions on RGB images while the red circles show the corresponding misaligned annotations.}
% \label{fig:rgb_mask_misalignment}
% \end{figure*}
% % \todos{don't mention anything that is not your contribution. just give reference.}

We leverage the ground truth plane mask from Plane-RCNN~\cite{Liu2019planercnn} which employs the 3D mesh reconstruction created from ScanNet~\cite{dai2017scannet} for the multi-plane instance proposals. Unfortunately, the plane annotations are noisy\footnote{Similar observations have been made by previous work~\cite{}.} as shown in Figure~\ref{fig:annotation_cleanup}.
% illustrates that the misaligned plane annotation the examp of RGB images on the top row and its corresponding masks extracted from Plane-RCNN on the bottom row.
%
% However, it is pointed out by the authors that the Plane-RCNN ground truth mask is not perfect, there are many cases where the 3D annotations projected onto the image are misaligned.
% %
% For example, in Figure~\ref{fig:rgb_mask_misalignment}, we show an example of RGB images on the top row and its corresponding masks extracted from Plane-RCNN on the bottom row.
%
The objects in the RGB images (dotted black box) are mis-aligned with their plane annotations. 
% The dotted circles show the position of objects in the RGB images, and the red circles show their corresponding annotated masks.
%
To detect mis-alignments, Plane-RCNN propose to compute the discrepancies between the depth from 3D mesh reconstruction and the corresponding depth map on the annotated regions.
%
While it is effective, it prunes a number of valid planes that are partially aligned with the RGB images.
%

Instead, we iterate a RANSAC~\cite{Fischler81} based plane fitting and region growing methods to refine the plane annotations. Given an annotated plane from Plane-RCNN, we fit a plane using the corresponding depth from ScanNet using a plane RANSAC with a strict inlier threshold (2 cm). This results in a small set of inliers due to noisy depth measurements. Given the initial inliers, we grow the coplanar region through neighboring pixels based on two criteria: (i) the distance from the 3D point to the plane is less than 20cm and (ii) the corresponding surface normal from FrameNet~\cite{Huang19FrameNet} is close to the plane normal (i.e., less than 30$^{\circ}$). If the plane is substantially smaller than the annotation, we discard the annotation. We iterate this process over annotated planes, which allows us to accurately compute the plane instances as shown in Figure~\ref{fig:annotation_cleanup}). With this process, the resulting annotated planes are well aligned with the RGB images. Our method is summarized in Algorithm~\ref{alg:plane_refining}.

% we can achieve a clean mask output that combine the feature of (i) the smooth 3D mesh reconstruction, (ii) the well-aligned of the depth map, and (iii) the identical surface normal over a plane mask, which is well-suited for supervising the surface normal prediction.



% \begin{figure}[h]
% \includegraphics[width=0.5\textwidth]{sections/figures/annotation_cleanup.png} 
% \centering
% \caption{Cleaning-up annotations: our method takes as input the depth, plane annotations, its surface normal in the first row. The following 4 rows showing the output of each step: Mask extractions, Planes fitting, Region growing and final output. The arrows indicate which input is used at each step.}
% \label{fig:annotation_cleanup}
% \end{figure}
%


% Our algorithm takes as input the annotated masks from Plane-RCNN, the depth map from ScanNet, and the normal map from FrameNet~\cite{Huang19FrameNet}.
% %

% In the mask extraction step, we examine each plane from the original annotations.
% %
% Next, in the plane fitting step, we use part of the depth map corresponding the examined plane mask and employ a RANSAC process to find the largest consensus that satisfies a plane equation (within a \textit{strict depth inlier threshold ($\alpha_{strict} = 2cm$)}.
% %
% This usually results in a smaller mask which contains many holes which is due to the noisy measurements of the depth map.
% %
% Finally, in the region growing step, we take that mask from the plane fitting step and grow out to its neighbouring pixels based on 2 criteria: (i) a relaxed depth inlier threshold ($\alpha_{relaxed}=20cm$) and (ii) the surface normal error (between the normal map and the plane mask's normal) is below a threshold ($\beta = 30^{\circ}$). 
% %
% Note that we also remove plane annotations that shrink substantially from the initial mask.
% %
% Using this technique, we can achieve a clean mask output that combine the feature of (i) the smooth 3D mesh reconstruction, (ii) the well-aligned of the depth map, and (iii) the identical surface normal over a plane mask, which is well-suited for supervising the surface normal prediction.
%
% Our method is summarized in Algorithm~\ref{alg:plane_refining}.

\begin{algorithm}[t]
  \caption{Refinement of plane annotation}
  \textbf{Input: } Plane instance mask from Plane-RCNN $\mathcal{M}_{\mathcal{I}}$, depth image from ScanNet $d_{\mathcal{I}}$, normal image from FrameNet $\mathbf{n}_{\mathcal{I}}$
  \textbf{Output: } Refined masks $\widetilde{\mathcal{M}}_{\mathcal{I}}$
  \begin{algorithmic}[1]
    \State set $\widetilde{\mathcal{M}}_{\mathcal{I}} = \emptyset$
    \For{$\mathcal{I}$ in $\mathcal{D}$}
    	\For{plane instance mask $m$ in  $\mathcal{M}_{\mathcal{I}}$}
      		\State $m_{\textsc{inlier}}$ = RANSAC plane fitting ($m$, $d_{\mathcal{I}}$)
      		\State $\tilde{m}$ = region grow($m_{\textsc{inlier}}$, $\mathbf{n}_{\mathcal{I}}$)
      		\If{ $ \frac{|\tilde{m}|}{m} > \delta$ }
        			\State Add $\tilde{m}$ to $\widetilde{\mathcal{M}}_{\mathcal{I}}$
      		\EndIf
      \EndFor
\EndFor
\State \Return $\widetilde{\mathcal{M}}_{\mathcal{I}}$
  \end{algorithmic}
  \label{alg:plane_refining}
\end{algorithm}
